Compositional Generalization with Tree Stack Memory Units

We study compositional generalization, viz., the problem of zero-shot generalization to novel compositions of concepts in a domain. Standard neural networks fail to a large extent on compositional learning. We propose Tree Stack Memory Units (Tree-SMU) to enable strong compositional generalization. Tree-SMU is a recursive neural network with Stack Memory Units (\SMU s), a novel memory augmented neural network whose memory has a differentiable stack structure. Each SMU in the tree architecture learns to read from its stack and to write to it by combining the stacks and states of its children through gating. The stack helps capture long-range dependencies in the problem domain, thereby enabling compositional generalization. Additionally, the stack also preserves the ordering of each node's descendants, thereby retaining locality on the tree. We demonstrate strong empirical results on two mathematical reasoning benchmarks. We use four compositionality tests to assess the generalization performance of Tree-SMU and show that it enables accurate compositional generalization compared to strong baselines such as Transformers and Tree-LSTMs.

==> abstract.tex <==
\begin{abstract}
% \aacomment{Generalization to harder problem instances (aka.. ) is challenging for standard neural networks. In contrast, recursive .. have the potential to achieve extrapolation. This is because .. However, recursive networks are prone to error propagation along trees of high depth and are unable to capture long range correlations effectively. To overcome this..}
Zero-shot generalization to harder compositional problem instances (a.k.a extrapolation) is challenging for standard neural networks. In contrast, recursive neural networks have the potential to achieve extrapolation because they are able to capture the compositionality of tree-structured data such as mathematical equations and program abstract syntax trees.
% , and hence, enable better generalization. 
However, in this paper we show that recursive networks are prone to error propagation along trees of high depth and are unable to capture long range dependencies effectively.
To overcome this, we propose \SMUlong s (Tree-SMUs), a novel memory augmented recursive neural network whose nodes consist of a differentiable stack.
% to increase the memory capacity of Tree-LSTMs.
% To overcome this, we propose a novel memory augmentation mechanism for recursive neural networks using a \emph{differentiable stack} embedded in LSTM cells of a Tree-LSTM. 
Each SMU cell learns to read from its stack and to write to it by combining the stacks and states of its children through gating.
% to increase the memory capacity of each node in the recursive structure using a differentiable stack. \aacomment{a novel memory augmentation mechanism to recursive networks using diff stack embedded in the LSTM cells}
% to augment each node in the recursive network with an external memory in the form of a differentiable stack. 
This architecture improves both the local and global representation of compositional data due to better expressive power and the ability to capture long-range dependencies by giving each node indirect access to its descendants. We demonstrate empirical results on four benchmark tasks across three domains 
% namely symbolic equation verification, equation completion, and addition, 
and show that Tree-\SMU~enables accurate extrapolation to significantly harder problem instances compared to strong baselines such as Transformers.
% Recursive neural networks are able to capture compositionality of tree-structured data such as mathematical equations, and hence, enable better generalization. However, generalization to harder problem instances (a.k.a extrapolation) is challenging. This is due to error propagation along the nodes of the recursive network and the inability to capture long-range dependencies effectively.

%representation at each node and global representations  by capturing long-range correlations in compositional data.

%due to two main problems, viz.,    imperfect learned representation in each node of   the recursive network and error propagation on as a result of the long range dependencies being forgotten as examples get more compositional and harder. In order to overcome these challenges, we propose to augment each node in recursive neural networks with a memory that has the data structure of a \emph{neural stack} with soft push and pop operations. We show that from a local perspective, the stack helps learn a better representation in each node and from a global perspective, the way the stack is structured allows each node to have access not only to its children but also its grand children, defeating error propagation. Our results indicate that the performance of memory augmented recursive neural networks is consistently better compared to the performance of recursive neural networks on harder examples that are not seen during training.
\end{abstract}

%%% old abstract:
%%%%%
% Recursive neural networks have shown an impressive performance for modeling compositional data compared to their recurrent counterparts. Although recursive neural networks are better at capturing long range dependencies, their generalization performance starts to decay as the test data becomes more compositional and potentially deeper than the training data. %\facomment{does this also hold for data of other distributions? What kinds of unseen composition complexities can our model handle? Is there a limitation on the type of composition complexity?}. 
% In this paper, we present memory-augmented recursive neural networks to address this generalization performance loss on deeper data points.
% %\facomment{maybe we should re-write the paper and claim that we are only generalizing this task}. 
% We augment Tree-LSTMs with an external memory, namely neural \emph{stacks}. We define soft push and pop operations for filling and emptying the memory to ensure that the networks remain end-to-end differentiable. In order to assess the effectiveness of the external memory, we evaluate our model on a neural programming task introduced in the literature called equation verification. Our results indicate that augmenting recursive neural networks with external memory consistently improves the generalization performance on deeper data points compared to the state-of-the-art Tree-LSTM by up to $10\%$.
% %\facomment{We should re-write the paper and claim that this is only for neural programming}

==> broader_impacts.tex <==
\section*{Broader Impact}
This paper focuses on the problem of extrapolating to harder data instances that is currently a challenge in the machine learning community.
% Extrapolation to harder problems is currently a challenge for neural networks. 
Addressing this problem is important in order to build models that can reason in complex scenarios by seeing examples of much lower complexity similar to humans. This can avoid overfitting to data which may be biased or imbalanced, and hence, leading to potentially more robust and fairer predictions.

Moreover, addressing the problem of extrapolation encourages models to be more sample efficient. Sample efficient models pave the way to Green Artificial Intelligence \cite{schwartz2019green} and help reduce the carbon footprint of deep learning research on the environment.
% reduce waste due to training large models for extended periods of time.

% It is important for models to be sample efficient since the compu
% We cannot think of an immediate negative societal outcome for this work.
%  Authors should discuss both positive and negative outcomes,
% if any. For instance, authors should discuss a) who may benefit from this research, b) who may be
% put at disadvantage from this research, c) what are the consequences of failure of the system, and d)
% whether the task/method leverages biases in the data. If authors believe this is not applicable to them,
% authors can simply state this.

==> dataStats.tex <==
% \begin{table*}[t]
%   \caption{\textbf{Data set statistics}}
% \label{tab:data}
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \multirow{2}{*}{\bf Statistic} & 
% 	\multicolumn{6}{c}{\bf Data depth}\\
% \cmidrule(lr){2-9}
%  & \bf all & \bf d=1 & \bf d=2 & \bf d=3 & \bf d=4 & \bf d=5 & \bf d=6 & \bf d=7  \\
% \midrule
% Number of equations & 50,573 & 39 & 2,547 & 12,217 & 15,034 & 13,007 & 5,980 & 1749  \\
% \addlinespace
% Correct portion & 55.53 & 25.64 & 43.82 & 53.29 & 48.86 & 61.91 & 64.72 & 67.52 \\
% \bottomrule
% \end{tabular}
% \end{table*}
\begin{table*}[t]
  \caption{\textbf{Data set statistics}}
\label{tab:data}
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{2}{*}{\bf Statistic} & 
	\multicolumn{14}{c}{\bf Data depth}\\
\cmidrule(lr){2-15}
 & \bf all & \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 & \bf 6 & \bf 7 & \bf 8 & \bf 9 & \bf 10 & \bf 11 & \bf 12 & \bf 13 \\
\midrule
Number of equations & 41,894 & 21 & 355 & 2,542 & 7,508 & 9,442 & 7,957 & 6,146 & 3,634 & 1,999 & 1,124 & 677 & 300 & 189  \\
\addlinespace
Correct portion & 0.56 & 0.52 & 0.57 & 0.62 & 0.61 & 0.58 & 0.56 & 0.54 & 0.52 & 0.52 & 0.49 &  0.50 & 0.50 & 0.50 \\
\bottomrule
\end{tabular}}
\end{table*}


==> depthTestTab.tex <==
\begin{table*}[t]
  \caption{\textbf{Generalization} to measure capability of the model to generalize to unseen depth. Acc, Prec and Rcl stand for accuracy, precision and recall, respectively. All the models are trained on equations of depth 1,2 and 3. The stack and queue capacity is 5.}
\label{tab:results}
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\bf Approach} & 
	\multicolumn{3}{c}{\bf Test depth: 4} & 
    \multicolumn{3}{c}{\bf Test depth: 5} & 
    \multicolumn{3}{c}{\bf Test depth: 6} &
    \multicolumn{3}{c}{\bf Test depth: 7} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}

 & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl\\
\midrule
Majority Class &  & - & -
&  & - & - 
&  & - & - \\
\addlinespace
TreeNN & $88.53\pm{0.19}$ & $83.27\pm{0.12}$ & $96.49\pm{0.03}$
& $89.95\pm{0.26}$ & $90.06\pm{0.17}$ & $94.18\pm{0.53}$
& $89.44\pm{0.25}$ & $90.40\pm{0.30}$ & $94.43\pm{0.33}$
& $90.13\pm{0.38}$ & $92.14\pm{0.42}$ &  $94.81\pm{0.47}$ \\
 TreeLSTM & $94.11\pm{0.09}$ & $90.17\pm{0.08}$ & $\bf 99.18\pm{0.03}$
&$95.31\pm{0.22}$ & $95.01\pm{0.16}$ & $\bf 98.18\pm{0.11}$
& $94.07\pm{0.11}$ & $93.11\pm{0.25}$ & $\bf 98.64\pm{0.06}$
& $93.63\pm{0.15}$ & $93.18\pm{0.25}$ & $\bf 98.67\pm{0.34}$ \\
 \addlinespace
 TreeNN + Queue & $88.54\pm{0.12}$ & $83.13\pm{0.17}$  & $96.76\pm{0.20}$ & $90.05\pm{0.32}$   & $90.62\pm{0.43}$  & $94.31\pm{0.15}$  & $89.70\pm{0.45}$  & $90.49\pm{0.36}$  & $94.56\pm{0.34}$ & $90.68\pm{0.11}$ & $92.74\pm{0.16}$ & $94.75\pm{0.45}$  \\
 TreeNN + Stack & $\bf 95.56\pm{0.35}$ & $\bf 92.90\pm{0.43}$ & $98.76\pm{0.16}$
& $\bf 95.37\pm{0.13}$ & $95.80\pm{0.42}$ & $97.32\pm{0.02}$
& $94.74\pm{0.09}$ & $95.06\pm{0.24}$ & $97.43\pm{0.30}$
& $\bf 94.95\pm{0.07}$ & $95.91\pm{0.25}$ & $97.1\pm{0.26}$  \\
 TreeNN + Stack + no-op & $95.26\pm{0.11}$ & $92.75\pm{0.27}$ & $98.62\pm{0.07}$
&\bf $95.51\pm{0.17}$ & $\bf 96.31\pm{0.32}$ & $97.32\pm{0.25}$
& $\bf 94.88\pm{0.22}$ & $\bf 95.52\pm{0.64}$ & $97.67\pm{0.13}$
& $94.38\pm{0.22}$ & $\bf 95.94\pm{0.35}$ & $96.64\pm{0.27}$\\
 TreeNN + Stack + top2 & $94.94\pm{0.09}$ & $92.00\pm{0.28}$ & $98.78\pm{0.09}$
& $95.33\pm{0.12}$ & $95.65\pm{0.11}$ & $97.59\pm{0.06}$
&$94.66\pm{0.21}$ & $94.59\pm{0.43}$ & $97.85\pm{0.25}$
& $94.66\pm{0.28}$ & $95.18\pm{0.42}$ & $98.08\pm{0.24}$\\
\bottomrule
\end{tabular}
}
\end{table*}


==> eq_completion.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/mrr_random_collapse.pdf}
    \caption{Mean reciprocal rank (MRR) }
    \label{fig:sample_eff}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/top1_random_collapse.pdf}
    \caption{Top\_1 Accuracy }
    \end{subfigure}
    \caption{Different metrics for equation completion. The plots show metric break-down with respect to the depth of the test equation.}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/top5_random_collapse.pdf}
    \caption{Top\_5 accuracy}
    \label{fig:sample_eff}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/top5_random_collapse.pdf}
    \caption{Equation Completion Experiment}
    \label{fig:sample_eff}
    \end{subfigure}
    \caption{Different metrics for equation completion. The plots show metric break-down with respect to the depth of the test equation.}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/top_1_collapse.pdf}
    \caption{Top\_1 accuracy non-random}
    \label{fig:sample_eff}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/top_5_collapse.pdf}
    \caption{Top\_5 accuracy non-random}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/top_10_collapse.pdf}
    \caption{Top\_10 accuracy non-random}
    \end{subfigure}
    \caption{Different metrics for equation completion. The plots show metric break-down with respect to the depth of the test equation.}
\end{figure}

==> global_view_figure.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}{
    \includegraphics[width=\textwidth]{figures/tree_lstm_simple.pdf}}
    \caption{Tree-LSTM}
    \label{fig:tree_TLSTM_simple}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}{
        \includegraphics[width=\textwidth]{figures/stack_lstm_simple.pdf}}
    \caption{Stack augmented Tree-LSTM}
    \label{fig:stack_LSTM_simple}
    \end{subfigure}
    \caption{Model architecture of Tree-LSTM vs. stack-augmented Tree-LSTM. The yellow symbol in Figure \ref{fig:model_TLSTMstack} represents the soft push/pop operation and it's details are shown in the square labeled soft push/pop. Both figures show a sub-tree with a parent block and its two children.}
    \label{fig:global_view}
\end{figure*}

==> introduction.tex <==
\section{Introduction}

% Systematic generalization (\facomment{define}) of neural networks has been a heavily debated topic since late 1980's \citep{fodor1988connectionism, smolensky1987constituent, marcus1998rethinking, marcus2019algebraic}. Recent work has shown mixed results about the systematic generalization ability of (mostly recurrent and flat) neural network architectures \citep{lake2018generalization, lample2019deep}. Recently \cite{bahdanau2018systematic} introduced a set of tasks that evaluate the systematic generalization ability of neural networks across several different dimensions (\facomment{not the best word?}). \facomment{actually instead of writing it this way, use this to motivate why we tackle this problem--rewrite}.

\facomment{old:}

Recurrent neural networks such as RNNs, LSTM, GRUs among other are popular neural networks used for modeling sequential data. The recently proposed Transformer architecture \citep{vaswani2017attention} and its variants \citep{devlin2018bert,radford2019language,brown2020language} have revolutionized the field of natural language processing. 

These language models have mostly been tested on natural language tasks. However, measuring systematicity in natural language it is not. Specifically, there is not a concrete definition of what systematic generalization in free-form open domain text is. There has been some initial studies on systematicity in natural language and how to measure it \citep{lake2018generalization,bahdanau2018systematic}, however, the tasks introduced by these studies typically simplifies natural language to a point where it is barely natural language and more code-like \facomment{better writing please}. We argue that systematic generalization abilities of neural networks can be more concretely evaluated in domain such as mathematics, logic and programming. For example, in the mathematics domain arbitrarily complex math expressions can be constructed using a limited number of base function. Same goes for the logic and programming domain. Therefore, one can generate a suite of generalization tasks to evaluate models on different aspects of systematicity \citep{bahdanau2018systematic}.

If there are compositional structures in the data, they can be leveraged to improve systematic generalization \facomment{write better}. For example, in mathematical or logical reasoning or program synthesis the data has an inherent hierarchical tree structure. Capturing that hierarchical structure in the neural network architecture allows for better generalization \citep{arabshahi2018combining,allamanis2017learning,evans2018can, shido2019automatic}.

In this paper, we propose Tree Stack Memory units (Tree-SMU) that ...

\begin{itemize}
    \item Systematic generalization is hard for neural networks
    \item When there is compositionality available in the data, we can improve systematic generalization by accounting for them
    \item When there is need for recursive function approximation we can use neural stacks to further improve systematic generalization -- why stacks? Why not other data structures?
    \item motivating example for error propagation: $2(x+y+z)-2z$
    \item flat recurrent neural networks completely ignore the systematicity and perform poorly. Transformers can hypothetically ``learn'' the compositionality. However, in practice we show that when the compositionality is available as supervision in the data, it is better to account for it directly in the network architecture.
    \item We design a set of compositionality tests suggested by \citet{hupkes2020compositionality} to test the systematic generalization of our proposed models.
    \item We show this result for the first time with the scale of tens of millions of data points. \textcolor{red}{We are not sure we can get these by the deadline}
    \item \textcolor{red}{Still open to debate:} How do we systematically test for recursion to empirically prove the effectiveness of stack?
\end{itemize}

Humans have impressive problem solving abilities. For example, in the context of mathematical problem solving, once they learn the concept of addition or multiplication, they are capable of applying them to unseen numbers with arbitrary (potentially infinite) compositionality. Are neural networks also capable of doing this? This question dates back to the 1980's and Fodor's statement \citep{fodor1988connectionism} about the incapability of neural networks to perform such compositional computations (a.k.a systematic compositionality). More recently, these claims were investigated for the task of semantic parsing in \citet{lake2018generalization} using a variety of recurrent neural networks (RNNs) with mixed results. They show that when the difference between the training and the test examples is small, RNNs generalize well to unseen examples. But when tasks require systematic compositional skills, RNNs fail spectacularly. An example of systematic compositionality is being able to successfully compute mathematical functions such as addition on an arbitrary number of inputs, and compose it with other functions like multiplication or division among others. %(being able to use primitive mathematical functions such as addition or multiplication in arbitrary complex equations and compute the results) 

More recently, similar results were shown in \citet{lample2019deep} for symbolic integration and solving differential equations using Transformers. Specifically, \citet{lample2019deep} showed that transformers have a near perfect performance when the training and test examples are from the same distribution. However, when they come from different distributions the performance significantly degrades and the transformer does not extrapolate to the test data. As stated in \citet{lample2019deep}, this is because the Transformer learns undesired behavior based on data artifacts such as the length of the input symbolic expression apart from learning the actual functionality of mathematical functions. % rather than the actual functionality of the primitive functions. %, dismissing the plausibility of using neural networks as a model of the mind
% \aacomment{we should address facebook paper head on here. Also say: subsequent to the release of this work, (to make to state we did first) transformers have much higher capability to capture long range correlations, but do not extrapolate, in fact, ... (mention how accuracy drops). make this another para}
In this paper, we show that accounting for the hierarchical structures in their data when encoding the equations enables us to significantly outperform the extrapolation performance of Transformers on the test data sets.

When the compositionality of the data is available as supervision (e.g. in mathematical and logical reasoning or program synthesis), tree-structured counterparts of RNNs, known as Tree-RNNs or recursive neural networks, drastically improve generalization to easy problems~\citep{tai2015improved, socher2011parsing, allamanis2017learning, evans2018can} and extrapolation to slightly harder problems \citep{arabshahi2018combining}. %\aacomment{and extrapolation much better, especially if test instances are of similar or only slightly higher tree depth}

In this paper, we show that the performance improvement of recursive neural networks has a fundamental limitation, when it comes to extrapolation to much harder instances compared to the training data. Specifically, we take the depth of the recursive structure (tree) as a metric for measuring the difficulty of a problem instance. We show that if we limit the depth of the training examples and test the trained recursive neural networks (such as Tree-RNN and Tree-LSTM) on unseen examples of much higher depth, then their performance decays rapidly with depth. % This was also shown in \cite{lake2018generalization} for RNNs.
% It is worth noting that as the tree depth grows, expressions also get longer
% inherent due to the correlation structures in tree-RNNs. The 
This limitation is due to error propagation along the tree and there are no error-correction mechanisms to overcome that.
% This performance degradation is primarily due to an imperfectly learned representation for the functions in the problem domain. This results in  error propagation along the tree. 

It is important to address this limitation since it is unreasonable to assume that the model has access to arbitrarily hard examples during training. Second, addressing the issue of extrapolation discourages the model from memorizing the training data and improves sample efficiency since the model can learn to exploit the algebraic compositionality of expressions similar to humans \citep{lake2018generalization}. %\aacomment{and we want to discourage just memorization}.
%this lack of generalization Second, \citet{lake2018generalization} argue that the sample inefficiency of neural networks, requiring large training datasets, suggests that models may lack the algebraic compositionality that humans exploit. Therefore, improving the generalizability of neural networks to unseen composition complexity also improves their sample efficiency.

% The problem of extrapolation (generalizing to harder instances) is especially important in neural programming. In this task, neural networks are used to learn programs, mathematics or logic from data~\citep{loos2017deep, allamanis2017learning,evans2018can,graves2014neural, zaremba2014learning,reed2015neural,cai2017making,saxton2019analysing}. Often in neural programming, a core neural network cell is used to learn and represent a certain program such as addition or sort and mathematical or logical function such as multiplication and OR. Neural programming is a suitable application for investigating the extrapolation capability of neural networks to harder problems because we can construct arbitrary complex expressions using a limited number of primitive functions.  \aacomment{i recommend just commenting this para  out. this is too late and out of place}

% The extrapolation performance of recursive neural networks degrades 
% The degradation in extrapolation performance of recursive neural networks is
% This performance degradation is primarily due to an imperfectly learned representation for the functions in the problem domain. This results in  error propagation along the tree. 
In order to address this limitation, we propose a novel Stack Memory Unit (\SMU) that increases the memory capacity of LSTM by replacing its memory with a differentiable \emph{stack}. The SMU node learns to control the read/write operations from/to its memory, and to propagate information along the tree. Our proposed Tree-SMU architecture
% reading from the top of the memory (pop) or writing to its memory top (push).
% augment recursive neural networks with an external memory in the form of a differentiable \emph{stack}. Each node in the tree has access to a unique stack and can either read its top element (pop) or write to its top element (push).
improves local and global errors and leads to a more robust extrapolation.

% \input{global_view_figure.tex}

% \aacomment{suggest moving these two paras before summary of results to later sections when u introduce stack augmentation. it is too long}
% From a local perspective, the stack structure encourages the model to learn a better representation for the functions. This is because most of these programs and functions can be implemented more compactly and efficiently using recursion, potentially making it easier for neural networks to model them. For example, the pseudo code for a recursive and non-recursive implementation of the multiplication function is given in Figure \ref{fig:mulFunc}. 
% % Another example of a symbolic representation of the recursive multiplication algorithm in Figure \ref{fig:mulFunc} is given below:
% % \begin{align}
% %     4 \times x & = x + 3 \times x \nonumber \\
% %     & = x + \big(x + (2 \times x)\big)  \label{eq:recMul} \\
% %     & = x + \big(x + (x+x)\big)
% %     \label{eq:example}
% % \end{align}
% % The compositional structure of Equation \ref{eq:recMul} is depicted in Figure \ref{fig:exampleEq}. 
% It is known that stacks are used to implement and execute a recursive function. Therefore, having access to a stack structure encourages the model to learn a better representation for each function.

% Second, the state of each node in a recursive neural network is computed using the states of its children. From a global perspective, stack enables each node to also have direct access to the state of its grand children by poping items from the stack. This helps the model to defeat error propagation by preserving values along the tree for longer.

% Neural programming refers to the task of using neural network to learn programs, mathematics and logic from data. Often in neural programming, a core neural network cell is used to learn and represent a certain program such as addition or sort and mathematical or logical function such as multiplication and OR. Most of these programs and functions can be implemented more compactly and efficiently using recursion, potentially making it easier for neural networks to model them. For example, the pseudo code for a recursive and non-recursive implementation of the multiplication function is given in Figure \ref{fig:mulFunc}. It is known that stacks are used to implement and execute a recursive function. 

% Compositional data are ubiquitous and  comopositional models are naturally the right candidates to fit such data. For example, recursive neural networks such as Tree-RNNs and Tree-LSTMs have been successfully applied to tasks in natural language processing, vision and neural programming \citep{tai2015improved,socher2011parsing,allamanis2017learning,arabshahi2018combining,evans2018can}. %In all these problems, data can be represented as a composition of its sub-components.

% Although recursive networks significantly outperform their flat counterparts, they still fail to generalize to unseen composition complexity. In other words, if we fix the composition complexity of the training data, the performance of the model decays significantly on test data of higher composition complexity which is mainly due to error propagation.

% Although recursive networks significantly outperform their flat counterparts, they still fail to generalize to unseen composition complexity. In other words, if we fix the composition complexity of the training data and test the models on unseen data points, the performance of the models start to decay as the complexity of the unseen data grows beyond that of the training data. This is an ongoing challenge for neural networks and it is important to address it because it is unreasonable to assume that the model sees all possible composition complexities during training. Therefore, it is important to build architectures that generalize to unseen composition complexity. \cite{lake2018generalization}
% \facomment{add a citation to NTM (potentially others that test on longer sequences). Since to the best of my knowledge no-one shows the failure on higher composition complexity, also draw a figure for a small problem and show that RNN, LSTM, (maybe an attention or memory baseline), treeRNN and treeLSTM decay in performance.}


% One of the reasons of this lack of generalization is error propagation as the composition complexity and depth grows. The more representative the components of the recursive neural network, the less the error propagation and the better the generalization performance to higher complexity. We show in this paper that external memory improves the generalization performance of recursive neural networks for neural programming.



% This behaviour is due to the absence of a fundamental component in the current state-of-the-art recursive neural network structures. This fundamental component is nothing but an internal stack or queue.
% % This behaviour is resulting from a fundamental concept that is currently missing from recursive neural networks and it is the concept of an external stack or queue.
% It is known that when traversing a recursive structure, algorithms typically use a stack or a queue to store information along the traversal path. However, the current state-of-the-art recursive neural networks such as Tree-LSTMs do not have access to such an external memory. Therefore their performance will be limited to a certain recursion depth, typically the depth seen in the training data.

% In order to show-case how this external memory structure helps recursive neural networks,
% consider the problem of representing mathematics and logic using recursive neural networks \citep{zaremba2014learning, allamanis2017learning, arabshahi2018combining, evans2018can}. Assume that our goal is to verify the correctness of the symbolic expression below using a recursive neural network such as a Tree-RNN.
% \begin{equation}
%     (x^0+2)+(1+(y^2+4)) = y^2 + 7
%     \label{eq:example}
% \end{equation}
% Assume that the Tree-RNN is rooted at equality (Figure \ref{fig:exampleEq}). Let us focus on how a Tree-RNN can equate the summation of the numbers $1,2$ and $4$ on the left-hand side of Equation \ref{eq:example} to number $7$ on the right-hand-side. If the output representation at node $\mathcal{A}$ is similar to the output representation of the right-hand-side, then the expression will be correctly classified. The output representation of $\mathcal{A}$ is computed from the representations of its direct children. This means that node $\mathcal{A}$ does not observe a fine-grained breakdown of the intermediate representations along the different depths of its sub-tree before computing the output representation. More specifically, as it is seen in Figure \ref{eq:example}, node $\mathcal{A}$ cannot directly access the numbers and operations in its two sub-trees, which in turn results in a distorted output representation that will negatively affect the model's performance. 

% In order to avoid this, we propose to augment each node with a stack that stores information about the nodes in its sub-tree. This stack is presented to the parent node and the parent can read from this stack directly as well as from the children. For example, the stacks of nodes $\mathcal{B}$ and $\mathcal{C}$ are shown in Figure \ref{fig:exampleEq}. node $\mathcal{A}$ now has direct access to it's children's stacks and produces a better output representation as a result.

% Note that contrary to a typical tree-traversal, we will be traversing the tree from the leaves to the root. Now assume that the recursion is currently at addition node $\mathcal{A}$ highlighted in red in Figure \ref{fig:exampleEq}. Node $\mathcal{A}$ takes as input the representation at each of its children and produces an output representation that represents the left-hand-side of Equation \ref{eq:example}. If all the sub-trees of $\mathcal{A}$ produced a perfect representation, then $\mathcal{A}$ would have also produced a perfect representation. However, this is not the case. Therefore, if $\mathcal{A}$ had access to the numbers in its sub-trees it would have produced a better output representation. We hypothesize that if each child node has a stack on which the information of its sub-tree traversal path is stored and $\mathcal{A}$ could access that stack when producing the output representation, then it will be able to produce a better informed output representation. In Figure \ref{eq:example}, $\mathcal{A}$ gets direct access to the number $2$ through node $\mathcal{B}$'s stack. 

% In this paper, we build upon this observation and intuition and introduce stack augmented recursive neural networks. We hypothesize that augmenting neural networks with additional stacks allows them to better represent recursive functions.
% We show that on the task of mathematical equation verification \citep{arabshahi2018combining} this structure consistently improves the generalization performance of Tree-LSTM on unseen (higher) depths. An example of a symbolic representation of the recursive multiplication algorithm in Figure \ref{fig:mulFunc} is given below:
% \begin{align}
%     4 \times x & = x + 3 \times x \nonumber \\
%     & = x + \big(x + (2 \times x)\big)  \label{eq:recMul} \\
%     & = x + \big(x + (x+x)\big)
%     \label{eq:example}
% \end{align}
% The compositional structure of Equation \ref{eq:recMul} is depicted in Figure \ref{fig:exampleEq}. In this paper, we use recursive neural networks for representing symbolic mathematical expressions where each function is a neural network whose weights are shared with the other appearances of that function.

% consider the problem of representing mathematics and logic using recursive neural networks \citep{zaremba2014learning, allamanis2017learning, arabshahi2018combining, evans2018can}. Assume that our goal is to verify the correctness of the symbolic expression below using a recursive neural network such as a Tree-RNN.

% We show that if we augment the cells of a recursive neural network with additional memory with the structure of a stack the cells are able to learn a better representation of the functions resulting in less error propagation and an improved generalization performance. 

% We also augment the cells with queues and show that stacks are a better choice for our task. This further reflects the fact that it is easier to implement recursive functions with stacks rather than queues.


% then the error caused by nodes farther from the root (red nodes) is more drastically propagated along the tree compared to the error from the nodes that are closer to the root. Therefore, if we store the representations of sub-trees and make them accessible to the parent nodes, they will have a higher chance of recovering from the error. 
% In order to do that we use the expression's parse tree to construct a Tree-RNN rooted at equality and predict the correctness of the equation at the root. The performance of such a model is highly dependent of the performance of the nodes farther from the root and if those nodes make a mistake in their output representations it is hard for the nodes close to the root to fix their mistake.
%  meaning that if a module is not behaving properly further down the tree, the higher nodes will not get a chance to fix their behavior and it will result in a performance loss. [very bad stence, fix]

% Moreover, whenever one traverses a recursive structure there is need to store information about the recursion path either using a stack or a queue.


% This is a major challenge for such models since this means that these models are ``memorizing'' the data rather than learning the underlying compsitionality and generalizing from it. Moreover, this suggests that these models are not capable of capturing longer range dependencies.

% In this paper, we address the challenge of generalizing to more complex compositions by augmenting Tree-RNNs with an external differentiable memory that the model can read from and write to. This will allow the model to put some of the burden of capturing long-range dependencies on the external memory, and instead focus on learning the underlying composition in the data. As a result, the model will be able to preserve longer range dependencies and generalize to data of unseen complexity.

% This additional capacity will allow the model to preserve longer range dependencies and ``remember'' data as we get farther and farther away from the leaves to the root. We will show that this will improve the performance of our model compared to powerful baselines such as Tree-LSTMs whose long short term memory capacity is developed for capturing long range dependencies \cite{tai2015improved}.

% The reason why we choose to augment recursive neural networks with both a stack and a queue is that depending on the application, one of them will be a better choice compared to the other. Therefore, one should pick either alternative based on their specific application. Stacks are naturally recursive data structures and suite problems that are recursive in nature, whereas queue is a better fit for serial data. For example, since mathematical equations are recursive, stack seems to be a better choice for it. [not sure about this analysis.]
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figures/example_recMul.pdf}
%     \caption{recursive symbolic multiplication of $4 \times x = x + \big(x + (2 \times x)\big )$}
%     \label{fig:exampleEq}
% \end{figure}
% \input{iterative_recursive.tex}
\input{modelFig.tex}
\vspace{-1em}
\subsection*{Summary of Results}
Our contributions in this paper are two-fold. First, we show that when there is compositional supervision available in the data, accounting for them significantly improves the model's zero-shot generalization ability compared to strong baselines such as Transformers. This is the first time that we show this result on data in the scale of 10's of millions of data points. Second, 
% The contributions of this paper are two-fold. First, we reveal a limitation of recursive neural networks: their lack of generalization to harder examples (extrapolation). Second, we propose to augment recursive neural networks with a differentiable memory that allows the model to extrapolate to harder instances for the task of learning and reasoning about mathematical equations. \aacomment{remove this.. too repetitive} %  This limitation was well-known for recurrent neural networks \cite{lake2018generalization}
% We increase the memory capacity of Tree-LSTMs by
we propose the Tree-Stack Memory Unit (Tree-SMU), which replaces the memory of a LSTM cell in a Tree-LSTM with a novel differentiable stack architecture. This architecture further improves the zero-shot generalization performance of state-of-the-art recursive neural networks to much harder problem instances. The \SMU~architecture is equipped with a trainable soft push and pop operator to read from and write to the stack. The stack is written to by combining the states and stacks of the children of each node, using a gating mechanism. As a result of this design, each node has indirect access to its descendants, resulting in error correction.
% This LSTM architecture has not been proposed before. \aacomment{how else have differentiable stacks been used before? clarify? we are not inventing stack. how is ours different from other neural models}
% augment Tree-RNNs and Tree-LSTMs with an external memory in the form of a differentiable stack. 
% We develop soft push and pop operations for the stack, and the model learns to control these operations. 
A stack is a Last In First Out (LIFO) data structure often used for recursive computation and implementation. Therefore, 
this model is ideal for applications that require modeling recursive functions. %To the best of our knowledge, stack-augmented LSTMs have not been proposed before.

% Due to the nature of these two data structures, the stack stores the local information of each sub-tree whereas the queue stores global information about the sub-tree of each node. Therefore, depending on the problem, one of these structures will be more suitable. For the case of mathematical equations, the stack structure is more suitable. We present a detailed discussion about this in the discussion section.
% The memory stores information about the traversal path of its sub-tree and provides this information to the parent node who will in turn produce a more informed output representation. We will also provide an analysis regarding how the memory is different from the memory of a tree-LSTM.
We test the proposed model on two neural programming tasks, (1) mathematical equation verification, where the goal is to verify the correctness of an input symbolic math equality, (2) mathematical equation completion, where the goal is to complete a blank in a given equality such that the equation holds \citep{arabshahi2018combining}, a differential equation solving task from \citet{lample2019deep} and a program synthesis task \citep{}. % and (3) Addition, where the goal is to test the model's ability to learn addition and is an evaluation of the counting ability of the model. 
These are good benchmarks for evaluating the proposed model because we can easily construct arbitrarily complex expressions by composing primitive functions and expressions to construct more complicated expressions.
% (Table \ref{tab:examples}, Appendix). 
%Moreover, many functions in this task can be implemented using recursion making the task an ideal test case for the proposed model. 
We show Tree-\SMU~consistently improves upon the extrapolation performance of Tree-RNN, Tree-LSTM and Transformers.
% to significantly harder problems on all tasks. %Moreover, we show that addressing extrapolation helps improve the sample efficiency of recursive neural networks, as we can achieve similar performance as Tree-LSTMs with 50\% of the data. 
Furthermore, we provide an ablation study that shows the effect of different model components on the final result. Lastly, we show that improving the extrapolation performance results in a better sample efficiency. \footnote{The code and data for re-producing all the experiments are available in the supplementary material, and will be released upon acceptance. We have also included a shell script that can be used to navigate the learned recursive model and the values stored in the stack}
% \aacomment{not a good place. put that in conclusion or in footnote} %We show that stack-augmented recursive neural networks consistently improve the \emph{extrapolation} performance of Tree-LSTMs and Tree-RNNs on the equation verification task.
% Moreover, we present a discussion about the stack's push and pop trace on a few examples and how they relate to the properties of different mathematical functions.

% In this paper, We present a novel method for increasing the capacity of recursive neural networks for better capturing long range dependencies. We propose to augment Tree-RNNs with an external memory with a stack and queue data structure. Our results indicate that this additional memory capacity will allow the network to generalize better to data of higher compositional complexity compared to powerful baselines such as Tree-LSTMs. We evaluate our model on a neural programming task called equation verification where given an input mathematical equation, our goal is to classify it as correct or incorrect. We represent composition complexity through the depth of the tree. Our experimental setup fixes the maximum depth of the training data and increases the depth of the test data. We observe that as the test data gets deeper, our model outperforms the baselines with a higher margin of up to about $\%3$ across different evaluation metrics. This indicates that the additional memory is preserving crucial information and propagating it along the tree to use at the time of decision making. We also perform an analysis of the model's performance across different queue and stack sizes.

%Recursive neural networks such as Tree LSTMS \cite{tai2015improved} and Tree NNs \cite{socher2011parsing} have shown promising results in modeling compositional data such as sentences that can be represented by parse trees, computer programs represented by their abstract syntax tree and mathematical equations \cite{zaremba2014learning, allamanis2017learning, arabshahi2018combining}. However, their performance degrades drastically when generalizing to expressions of higher depth. This suggests that information might be lost as it propagates from the leaves to the tree root. Therefore, we propose augmenting these networks with additional memory to overcome this issue.

% One line of work explores the possibility of providing random access operations such as reading from and writing to a memory or key-value pair access to the memory \cite{graves2014neural,reed2015neural,cai2017making}. Our work is inspired by the previous efforts that augment recurrent neural networks with stacks and queues \cite{das1992learning,sun2017neural,joulin2015inferring,grefenstette2015learning} where continuous push and pop operations are learned based on a

% \cite{das1992learning, weston2015,joulin2015inferring,grefenstette2015learning} .Inspired by these works, we present to augment recursive neural networks with differentiable data structures such as stacks and queues

% Inspired by the recent work on augmenting neural networks with abstract queues and stacks \cite{grefenstette2015learning, sun2017neural, joulin2015inferring,weston2015, kumar2016ask, sukhbaatar2015end,graves2014neural} we propose to augment recursive neural networks such as Tree-NNs and Tree-LSTMs \cite{tai2015improved} with external differentiable memory such as neural stacks and queues. 

% Memory networks and their differentiable counterpart \cite{weston2015, sukhbaatar2015end} store instances of the input data into an external memory that can later be read through their recurrent neural network architecture. This is different from enabling a model to read and write to an external memory such as a stack and a queue and limits the applicability of the model to scenarios where such paris can indeed be stored in the memory.

% Reed et al, and Cai et al propose key-value pair style memory \cite{reed2015neural,cai2017making}




==> iterative_recursive.tex <==
% \begin{minipage}{\linewidth}
\begin{figure}[h]
% \begin{lstlisting}[style=customPython, caption={non-recursive vs. recursive multiplication of numbers $x$ and $y$ in base 10.}, label={lst:mulFunc}]
% commentstyle=\fontseries{lc}\selectfont\itshape,columns=fullflexible
\begin{subfigure}{0.48\textwidth}
\begin{lstlisting}[style=customPython]
# Iterative multiplication
def mul(x, y):
  # x and y are lists of digits with 
  # the least significant bit in index 0
  prod = zeros(1,len(x)+len(y)-1)
  for x_i in range(0,len(x)):
    carry = 0
    for y_i in range(0,len(y)):
      prod[x_i+y_i] += carry + x[x_i] * y[y_i]
      carry = prod[x_i+y_i] / 10.0
      prod[x_i+y_i] = prod[x_i+y_i] mod 10.0
    prod[x_i+len(y)-1] = carry
  return prod
  
# Recursive multiplication
def recursive_mul(x,y):
  if x<y:
    return recursive_mul(y,x)
  elif y != 0:
    return (x + recursive_mul(x, y-1))
  else:
    return 0
\end{lstlisting}
% \end{minipage}
\caption{Multiplication Implementations}
\label{fig:mulFunc}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
% \centering
    \includegraphics[width=\textwidth]{figures/example_recMul.pdf}
    \caption{Symbolic Multiplication}
    \label{fig:exampleEq}
\end{subfigure}
\caption{Fig~\ref{fig:mulFunc}: non-recursive vs. recursive multiplication of numbers $x$ and $y$ in base 10. As can be seen, the recursive implementation is more compact. Note that if $x$ and $y$ are floating point numbers they should first be pre-processed and converted into integers through multiplication and the result should be converted back to floating point through division. Fig~\ref{fig:exampleEq}: recursive symbolic multiplication of $4 \times x = x + \big(x + (2 \times x)\big )$}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figures/example_recMul.pdf}
%     \caption{recursive symbolic multiplication of $4 \times x = x + \big(x + (2 \times x)\big )$}
%     \label{fig:exampleEq}
% \end{figure}
% \input{iterative_recursive.tex}
% \input{modelFig.tex}

==> localismTable.tex <==
% --- Localism Experiments Results ---
\begin{table}[t]
\centering
  \caption{\textbf{Localism Test} Equation Verification, Overall model Accuracy on train and test datasets}
\label{tab:localism}
\resizebox{0.6\textwidth}{!}{%
\centering
\begin{tabular}{lccc}
\toprule 
\textbf{Approach} & 
	\textbf {Train (Depths 1-7)} & 
	\textbf {\bf Validation (Depths 1-7)} & 
    \textbf {\bf Test (Depths 8-19)} \\
% \cmidrule(lr){2-4}
% \cmidrule(lr){5-7}
% \cmidrule(lr){8-10}
%  & \bf Acc & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl \\
\midrule
% Majority Class &  58.12 & 56.67 & 51.71 \\
% \addlinespace
% LSTM & 85.62 & 
% 79.48$\pm{4.53}$
% & 68.36$\pm{0.42}$ \\
% Transformer & 81.26 & 76.45$\pm{0.42}$
% & 61.05$\pm{1.53}$ \\
% Tree Transformer & 84.08 & 77.80$\pm{0.46}$
% & 62.12$\pm{1.06}$ \\

\addlinespace
Tree-RNN & $99.07 \pm{0.31}$ & $88.33 \pm{0.37}$  & $85.36\pm{0.35}$ \\
Tree-LSTM & $99.79 \pm{0.02}$ & $91.70\pm{0.0.28}$
 & $91.58\pm{0.11}$ \\
\addlinespace
Tree-SMU & $95.04 \pm{0.07}$ & $92.78\pm{0.09}$ & $\mathbf{98.86\pm{0.07}}$ \\
\bottomrule
\end{tabular}
}
\end{table}

==> localism_tests_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Tree-SMU/ICLR/figures/localism_test_depth_breakdown.pdf}
    \caption{\textbf{Localism Test} breakdown of model accuracy across different depths for baselines Tree-RNN and Tree-LSTM}
    \label{fig:localism_figure}
\end{figure}

==> results_sample_plot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.1\columnwidth]{figures/sampleEfficiency.pdf}
    \caption{Sample efficiency - The percentage in the legend indicates the percentage of the training data that is used for training each model.}
    \label{fig:sample_eff}
\end{figure}

==> sizeFig.tex <==
\begin{figure}
    \centering
    % \begin{subfigure}{0.45\textwidth}{
    \centering
    \includegraphics[width=0.8\textwidth]{figures/stackSize.pdf}
    \caption{The effect of different stack sizes on the performance of the Tree-RNN+stack model}
    \label{fig:stackSize}
    \end{figure}
    \begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/queueSize.pdf}
    \caption{The effect of different queue sizes on the performance of the Tree-RNN+queue model}
    \label{fig:QueueSize}
    % \end{subfigure}
\end{figure}

==> stackSizeTab.tex <==
\begin{table}[t]
  \caption{\textbf{Stack Size} to assess performance of the model with different stack sizes.}
\label{tab:gen}
\centering
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{\bf Tree-RNN + Stack} & 
	\multicolumn{3}{c}{\bf Stack size: 3} & 
    \multicolumn{3}{c}{\bf Stack size: 4} & 
    \multicolumn{3}{c}{\bf Stack Size: 10} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
 & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl \\
\midrule
Test depth 4   
& 92.22 & 88.79 & 94.51 
&  92.43&88.86 & 95.13&  92.88& 89.65 & 95.13\\
Test depth 5  
 & 87.16 & 86.11 & 93.53 & 87.87 &  87.70 &92.51&87.70 & 86.60  &93.90 \\
Test depth 6  
 & 82.76 & 89.19 & 94.56 & 82.84 & 89.88 &93.67 &82.40 & 87.70 & 95.78\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[t]
  \caption{\textbf{Queue Size} to assess performance of the model with different queue sizes.}
\label{tab:gen}
\centering
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{\bf Tree-RNN + Queue} & 
	\multicolumn{3}{c}{\bf Queue size: 3} & 
    \multicolumn{3}{c}{\bf Queue size: 4} & 
    \multicolumn{3}{c}{\bf Queue Size: 10} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
 & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl & \bf Acc & \bf Prec & \bf Rcl \\
\midrule
Test depth 4   
&92.92 & 89.67 & 95.29 & 92.47 & 89.14 & 94.67 & 93.10 & 90.29 & 94.82 \\
Test depth 5  
& 87.99 & 87.35 & 92.96 & 87.53 & 86.30 & 97.08 & 88.64 & 88.20 & 97.51 \\
Test depth 6  
 & 83.27 & 89.55 & 94.86 & 84.58 & 92.38 & 97.27 & 84.14 & 91.24 & 97.27 \\
\bottomrule
\end{tabular}
\end{table}
